SMT-Based Safety Verification of Data-Aware Processes under Ontologies (Extended Version)

In the context of verification of data-aware processes (DAPs), a formal approach based on satisfiability modulo theories (SMT) has been considered to verify parameterised safety properties of so-called artifact-centric systems. This approach requires a combination of model-theoretic notions and algorithmic techniques based on backward reachability. We introduce here a variant of one of the most investigated models in this spectrum, namely simple artifact systems (SASs), where, instead of managing a database, we operate over a description logic (DL) ontology expressed in (a slight extension of) RDFS. This DL, enjoying suitable model-theoretic properties, allows us to define DL-based SASs to which backward reachability can still be applied, leading to decidability in PSPACE of the corresponding safety problems.

==> 10.1_dlite.tex <==
\subsection*{Proofs for Section~\ref{sec:prel}}
%{$\DLitebn$ Equisatisfiable Universal FO$^1$ Translation}

%The proof of Lemma~\ref{lem:dlfoequiv} is standard~\cite{BaaEtAl03}.
%To show Lemma~\ref{lem:dlitefoequisat},
Following~\cite{ArtEtAl09}, we define a polynomial translation of a $\DLitebn$ ontology $\Omc = (\Tmc, \Amc)$ into an equisatisfiable universal FO$^1$ formula $T(\Omc)$.
%\ldots
%\nb{M: working here}
Let $\NI(\Omc)$ be the set of individual names occurring in $\Omc$. Moreover, $\NR(\Omc)$ is the set of role names occurring in $\Omc$, while $\role(\Omc) = \NR(\Omc) \cup \{ P^{-} \mid P \in \NR(\Omc) \}$, and let $\con{\Omc}$ be the set of concepts occurring in $\Omc$.
%is the set of all role occurring in $\Omc$ together with their inverses.
Given a $\DLitebn$ concept $C$, the FO$^{1}$ formula $C^{*}(x)$ is defined inductively as follows:
%
\begin{gather*}
	A^* = A(x), \quad
	\bot^* =\bot, \quad
	(\mathop{\geq q} R)^* = E_qR(x), \\
	(\neg D)^* = \neg D^* \quad
	(D \sqcap E)^* = D^* \land  E^*,
\end{gather*}
%
For the TBox $\Tmc$, we define the FO$^1$ sentence
%
\begin{equation*}
\Tmc^{\ddagger} = \bigwedge_{C \sqsubseteq D \in \Tmc} \forall x \bigl{(} C^{*} \to D^{*} \bigr{)}.
\end{equation*}
%
We denote by $Q_{\Tmc}$ the set containing $1$ and the numerical parameters of the number restrictions occurring in $\Tmc$, i.e.,
%
\begin{equation*}
Q_{\Tmc} =  \{ 1 \}  \cup  \{ q \mid \mathop{\geq q} R \ \text{occurs in} \ \Tmc \}.
\end{equation*}
%
Moreover, for each role name
$P_{k} \in \NR(\Omc)$,
%$P_{k} \in \role(\Omc)$,
we consider a pair of individual names $\mathit{dp_{k}}$ and $\mathit{dp^{-}_{k}}$,
and let
$\mathit{dr}(\Omc) = \{ \mathit{dr} \mid R \in \role(\Omc) \}$.
We then define
\nb{M: to check}
%
\begin{align}
	\label{eq:role:existence:2}
 	&
		 \delta(R) = 
%		 \bigwedge_{R \in \role(\Omc)}
	\bigwedge_{\substack{q, q' \in Q_{\Tmc} \\ q < q'}}
%  \\ \lnot \exists q'' \in Q_\T \colon q < q'' < q'}
	\forall x\bigl{(} (\mathop{\geq q'}R)^{*} \to (\mathop{\geq q}R)^{*} \bigr{)}, \\
 	&
	\varepsilon(R) = 
%	\bigwedge_{R \in \role(\Omc)} 
	\forall x \Bigl((\geq 1 R)^* \rightarrow \inv{\bigl((\geq 1 {R})^*(\mathit{dr})\bigr)} \Bigr).
	\label{eq:role:saturation}
%
\end{align}
where
$\inv{\bigl((\geq 1 {R})^*(\mathit{dr})\bigr)} = (\geq 1 {P^{-}_{k}})^*(\mathit{dp^{-}_{k}})$, if $R = P_{k}$, and $\inv{\bigl((\geq 1 {R})^*(\mathit{dr})\bigr)} = (\geq 1 {P_{k}})^*(\mathit{dp_{k}})$, if $R = P^{-}_{k}$.
%\nb{M: todo fix}
%$\inv{R}$ is the inverse of $R$, i.e., $\inv{P} = P^-$ and $\inv{P^-} = P$, for $P \in \NR(\Omc)$.
%
In addition, the translation of the
%$\DLitebn$
ABox $\Amc$ is
defined as
\nb{M: to check}
%
\begin{equation*}
  \Amc^{\ddagger} = \bigwedge_{A(a) \in \Amc} A(a) \land \bigwedge_{\neg A(a)\in \Amc} \neg A(a) \land \bigwedge_{R(a,b)\in \Amc} (\mathop{\geq q^{R, a}_{\Amc}} R)^*(a) \land \bigwedge_{\substack{\neg R(a,b) \in \Amc, \\ R(a,b) \in \Amc }} \hspace{-0.5cm} \bot,
\end{equation*}
%
where $\smash{q^{R, a}_{\Amc}}$ is the number of distinct $R$-successors of $a$
in $\Amc$, that is
%\emph{since we adopt the UNA}:
%
\begin{equation*}
  q^{R,a}_{\Amc} = \max \{ q \in Q_{\Tmc}
  \mid R(a,b_1),\dots,R(a,b_q)\in\Amc, \ \text{for distinct} \ b_1, \ldots, b_q \}.
\end{equation*}
%
Finally, we set
\[
	T(\Omc) = \Tmc^{\ddagger} \land \Amc^{\ddagger} \land  \bigwedge_{R \in \role(\Omc)} \big(\delta(R) \land \varepsilon(R)\big).
\]
%
%Lemma~\ref{lem:dlitefoequisat} follows immediately from the statement below.

%\begin{lemma}
\dliteequisat*
%A $\DLitebn$ ontology $\Omc$ is satisfiable with the UNA iff the universal FO$^1$ sentence $T(\Omc)$ is satisfiable.
%\end{lemma}
\begin{proof}

$(\Rightarrow)$
Assume that $\Omc$ is satisfiable (under the UNA), and let $\Imc = (\Delta^{\Imc}, \cdot^{\Imc})$ be a DL interpretation (that respects the UNA) such that $\Imc \models \Omc$.
%
We define an FO interpretation $\Jmc = (\Delta^{\Jmc}, \cdot^{\Jmc})$ as follows.
\nb{M: to check}
We set
$\Delta^{\Jmc} = \Delta^{\Imc}$.
Individual names are interpreted in the following way:
for $a \in \NI(\Omc)$, $a^{\Jmc} = a^{\Imc}$;
for every $R \in \role(\Omc)$, $\mathit{dr}^{\Jmc} = d$, with $d \in (\geq 1 R)^{\Imc}$, if $(\geq 1 R)^{\Imc} \neq \emptyset$, and $d$ arbitrary otherwise;
other individual names in $\NI$ are interpreted arbitrarily.
For predicate symbols, we set the following:
for $A \in \NC$, $A^{\Jmc} = A^{\Imc}$; for $R \in \role(\Omc)$ and $q \in Q_{\Tmc}$, $E_{q}R^{\Jmc} = (\geq q R)^{\Imc}$;
\nb{M: to check}
for $P \in \NR(\Omc)$, $P^{\Jmc} = P^{\Imc}$;
other predicate symbols in $\NPr$ and function symbols in $\NF$ are interpreted arbitrarily.
%
%\begin{itemize}
%	\item $\Delta^{\Jmc} = \Delta^{\Imc}$;
%	\item for individual names in $\NI$:
%	\begin{itemize}
%		\item for $a \in \NI(\Omc)$, $a^{\Jmc} = a^{\Imc}$;
%		\item for every $R \in \role(\Omc)$, $\mathit{dr}^{\Jmc} = d$, with $d \in (\geq 1 R)^{\Imc}$, if $(\geq 1 R)^{\Imc} \neq \emptyset$, and $d$ arbitrary otherwise;
%		\item other individual names in $\NI$ are interpreted arbitrarily;
%	\end{itemize}
%	\item for $A \in \NC$, $A^{\Jmc} = A^{\Imc}$; for $R \in \role(\Omc)$ and $q \in Q_{\Tmc}$, $E_{q}R^{\Jmc} = (\geq q R)^{\Imc}$;
%	\item for $R \in \role(\Omc)$, $R^{\Jmc} = R^{\Imc}$;
%	\item other predicate symbols in $\NPr$ and function symbols in $\NF$ are interpreted arbitrarily.
%%	\item for every $R \in \role(\Omc)$ and every pair $a, b \in \NI(\Omc)$, 
%\end{itemize}	
%
It can be seen (cf.~\cite{ArtEtAl09})
\nb{M: to check}
that $\Jmc \models T(\Omc)$.

$(\Leftarrow)$
Suppose that $T(\Omc)$ is satisfiable, and consider a model $\Jmc = (\Delta^{\Jmc}, \cdot^{\Jmc})$ of $T(\Omc)$ such that, without loss of generality~\cite{ArtEtAl07,ArtEtAl09},
\nb{M: to check}
$\Delta^{\Jmc} = \NI(\Omc) \cup \mathit{dr}(\Omc)$
%$\Delta^{\Jmc}$
%is countable and $a^{\Jmc}$ are all distinct, for $a \in \NI(\Omc)$
(i.e., $\Jmc$ is an Herbrand model of $T(\Omc)$,  see for instance~\cite{Rau06} for details, where the domain consisting of all the constants that occur in $T(\Omc)$).
We set
\nb{M: to check}
$\Delta_{0} = \Delta^{\Jmc}$,
%$\Delta_{0} = \{ a^{\Jmc} \mid a \in \NI(\Omc) \} \subseteq \Delta^{\Jmc}$,
and we will construct inductively
%a sequence of sets $\Delta_{m}$, ordered by inclusion, to define
a DL interpretation $\Imc = (\Delta^{\Imc}, \cdot^{\Imc})$ with domain $\Delta^{\Imc} = \bigcup_{m \leq 0} \Delta_{m}$, so that
$\Delta_{m} \subseteq \Delta_{m+1}$, for $m \leq 0$.
%
\nb{M: to check}
Each $\Delta_{m+1}$, for $m \leq 0$, is constructed from $\Delta_{m}$ by adding to it some fresh \emph{copies} of certain elements of
$\Delta_{0}$,
%$\Delta^{\Jmc} \setminus \Delta_{0}$:
%
so to have a function
$\mathit{cp} : \Delta^{\Imc} \longrightarrow \Delta_{0}$
such that
$\mathit{cp}(u') = u$, if such a new element $u'$ is a copy of
$u \in \Delta_{0}$
%$u\in \Delta^{\Jmc} \setminus \Delta_{0}$;
and
$\mathit{cp}(u) = u$, if $u \in \Delta_{0}$.
%we set $\mathit{cp}(u) = u'$, if such a new element $u$ is a copy of $u' \in \Delta^{\Jmc} \setminus \Delta_{0}$; and we set $\mathit{cp}(u) = u$, if $u \in \Delta^{\Jmc}$.

For individual names $a \in \NI$, we set $a^{\Imc} = a^{\Jmc} \in \Delta_{0} \subseteq \Delta^{\Imc}$.
%
For concept names $A \in \NC$, we set $A^{\Imc} = \{ u \in \Delta^{\Imc} \mid \Jmc \models A^{\ast}[\mathit{cp}(u)] \}$.
%
The construction of the interpretation of role names $P_{k} \in \NR$, together with the domain $\Delta^{\Imc}$, is as follows. We will take
\[
P_{k}^{\Imc} = \bigcup_{m \geq 0} P_{k}^{m}
\]
where $P_{k}^{m} \subseteq \Delta_{m} \times \Delta_{m}$, for every $m \geq 0$.
%
To define such $P_{k}^{m}$, we define the \emph{required $R$-rank of $d \in \Delta^{\Jmc}$}, as $r(R,d) = \max(\{ 0 \} \cup \{ q \in Q_{\Tmc} \mid \Jmc \models E_{q}R[d] \})$.
%
Since $\Jmc \models \delta(R)$, for every $R \in \role(\Omc)$, we have that $r(R,d)$ is a function, and that $r(R,d) = q$ implies $\Jmc \models E_{q'}R[d]$, for every $q' \in Q_{\Tmc}$ such that $q' \leq q$, and $\Jmc \models \lnot E_{q''}R[d]$, for every $q'' \in Q_{\Tmc}$ such that $q'' \geq q$.
%
We also define the \emph{actual $R$-rank of $d \in \Delta^{\Imc}$ at step $m$} as
\[
r_{m}(R, w) =
\begin{cases}
| \{ w' \in \Delta_{m} \mid (w, w') \in P_{k}^{m} \} |, & \text{if $R = P_{k}$}; \\
| \{ w' \in \Delta_{m} \mid (w', w) \in P_{k}^{m} \} |, & \text{if $R = P^{-}_{k}$}. \\
\end{cases}
\]
%\max(\{ 0 \} \cup \{ q \in Q^{R}_{\Tmc} \mid ( \})$
We then set $P_{k}^{{0}} = P^{\Jmc} \cup \{ (a^{\Imc}, b^{\Imc}) \in \Delta_{0} \times \Delta_{0} \mid P_{k}(a,b) \in \Amc \}$.
%
%By definition of $\Amc^{\ddagger}$, for every $R \in \role(\Omc)$ and $u \in \Delta_{0}$, we have that
%\nb{M: to check}
%\begin{equation}
%r_{0}(R, u) \leq r(R, \mathit{cp}(d))
%\end{equation}
%
Suppose now that $\Delta_{m}$ and $P_{k}^{m}$ have been defined, for $m \geq 0$.
Given a role name $P \in \role(\Omc)$, we define the following two sets of \emph{defects in $P^{m}_{k}$}:
\[
	\Lambda^{m}_{R} = \{ u \in \Delta_{m} \setminus \Delta_{m-1} \mid r_{m}(R, u) < r(R,u) \},
\]
where $R \in \{ P_{k}, P^{-}_{k} \}$ and we set $\Delta_{-1} = \emptyset$.
%
We then extend $\Delta_{m}$ and $P^{m}_{k}$ to $\Delta_{m+1}$ and $P^{m+1}_{k}$, respectively, according to the following rules:

\begin{enumerate}
%
	\item[$(\Lambda^{m}_{P_{k}})$] Let $u \in \Lambda^{m}_{P_{k}}$, $d = \mathit{cp}(u)$ and $q \in r(P_{k}, u) - r_{m}(P_{k}, u)$. We have that $\Jmc \models E_{q'}P_{k}[d]$, for some $q' \geq q > 0$. Since $\Jmc \models \varepsilon(R)$, for every $R \in \role(\Omc)$, we obtain $\Jmc \models E_{1}P_{k}[d]$, and given that $\Jmc \models \delta(R)$, for every $R \in \role(\Omc)$, we have $\Jmc \models E_{1}P_{k}^{-}[dp_{k}^{-}]$. Then, take $q$ fresh copies $u'_{1}, \ldots, u'_{q}$ of $dp_{k}^{-}$, setting $\mathit{cp}(u'_{i}) = dp^{-}_{k}$, for $1 \leq i \leq q$, add $u'_{i}$, for $1 \leq i \leq q$, to $\Delta^{m+1}$, and add the pairs $(u, u'_{i})$, for $1 \leq i \leq q$, to $P^{m+1}_{k}$.
	%
	\item[$(\Lambda^{m}_{P_{k}^{-}})$] Let $u \in \Lambda^{m}_{P^{-}_{k}}$, $d = \mathit{cp}(u)$ and $q \in r(P^{-}_{k}, u) - r_{m}(P^{-}_{k}, u)$. We have that $\Jmc \models E_{q'}P^{-}_{k}[d]$, for some $q' \geq q > 0$. Since $\Jmc \models \varepsilon(R)$, for every $R \in \role(\Omc)$, we obtain $\Jmc \models E_{1}P^{-}_{k}[d]$, and given that $\Jmc \models \delta(R)$, for every $R \in \role(\Omc)$, we have $\Jmc \models E_{1}P_{k}[dp_{k}]$. Then, take $q$ fresh copies $u'_{1}, \ldots, u'_{q}$ of $dp_{k}^{-}$, setting $\mathit{cp}(u'_{i}) = dp_{k}$, for $1 \leq i \leq q$, add $u'_{i}$, for $1 \leq i \leq q$, to $\Delta^{m+1}$, and add the pairs $(u'_{i}, u)$, for $1 \leq i \leq q$, to $P^{m+1}_{k}$.
	%
\end{enumerate} 

One can now show the following claims, the proof of which is analogous to the one given in~\cite{ArtEtAl09}.

\begin{claim}
For every $R \in \role(\Omc)$, $q \in Q_{\Tmc}$ and $u \in \Delta^{\Imc}$, $\Jmc \models E_{q}R[\mathit{cp}(u)]$ iff $u \in (\geq q R)^{\Imc}$.
\end{claim}
%\begin{proof}
%Cf.~\cite{ArtEtAl09}.
%\end{proof}

\begin{claim}
For every concept $C \in \con{\Omc}$ and $u \in \Delta^{\Imc}$, $\Jmc \models C^{\ast}[\mathit{cp}(u)]$ iff $u \in C^{\Imc}$.
\end{claim}
%\begin{proof}
%Cf.~\cite{ArtEtAl09}.
%\end{proof}

%Thanks to the claims above and following the proofs in~\cite{ArtEtAl09}, 

\begin{claim}
$\Imc \models \Tmc$ 
and
$\Imc \models \Amc$.
\end{claim}
%\begin{proof}
%Cf.~\cite{ArtEtAl09}.
%\end{proof}

The previous claim means that $\Imc \models \Omc$, as required.
\qedhere
\end{proof}

==> useful-material.tex <==
%\subsection{Model Checking over DB schemata}
%\label{app_sec2}






\begin{proposition}\cite{MSCS20}\label{prop:mc} A DB theory
	 $T$ has decidable constraint satisfiability problem and admits a model completion in  case it is axiomatized by finitely many universal one-variable formulae and $\Sigma$ is acyclic. 
	 %\begin{itemize}
	 % \item[{\rm (i)}] $\Sigma$ is acyclic and $T$ has the amalgamation property;
	 % \item[{\rm (ii)}] $T$ is empty or contains any subset of the above axioms~\eqref{eq:null}-\eqref{eq:null2}.\footnote{Da controllare.  }
	 %\end{itemize}
         %
	\end{proposition}
%
%	\begin{proof}
%	 See the Appendix.
%	\end{proof}




\begin{proof} 

First, notice that, in case $\Sigma$ is acyclic, $T$ has the finite model property. In fact, if $T:=\emptyset$, then congruence closure ensures that the finite model property holds and decides  constraint satisfiability in time $O(n\log n)$. Otherwise, we reduce the argument to the Herbrand Theorem.  Indeed, suppose to have a finite set $\Phi$ of universal formulae
%
and let $\phi(\ux)$ be the constraint we want to test for satisfiability. Replace the variables $\ux$ with free constants $\ua$. Herbrand Theorem states that $\Phi\cup \{\phi(\ua)\}$ has a model iff the set of ground $\Sigma^{\ua}$-instances of $\Phi\cup \{\phi(\ua)\}$ has a model. These ground instances are finitely many by acyclicity, so we can reduce to the case where $T$ is empty. Hence,  the constraint satisfiability problem for $T$ is decidable.

%
To show the existence of a model completion,
we freely take inspiration from an analogous result in~\cite{wheeler,LIP} and we  preliminarily show that $T$ is amalgamable. 

Let $\cM_1$ and $\cM_2$ two models of $T$ with a submodel $\mathcal{M}_0$ of $T$ in common (we suppose for simplicity that $|\cM_1|\cap|\cM_2|=|\cM_0|)$. We define a $T$-amalgam $\cM$ of $\cM_1, \cM_2$ over $ \cM_0$ as follows (we use in an essential way the fact that $\Sigma$ contains only \textit{unary} function symbols and $n$-ary relation symbols). 
Let the support of $\cM$ be the set-theoretic union of the supports of $\cM_1$ and $\cM_2$, i.e. $|\cM|:= |\cM_1|\cup |\cM_2|$. $\cM$ has a natural $\Sigma$-structure inherited by the $\Sigma$-structures $\cM_1$ and $\cM_2$.
%
For every function symbol $f$ in $\Sigma$, we define, for each $m_i\in |\cM_i|$ ($i=1,2$), $f^{\cM}(m_i):=f^{\cM_1}(m_i)$, i.e. the interpretation of $f$ in $\cM$ is the restriction of the interpretation of $f$ in $\cM_i$ for every element $m_i\in |\cM_i|$. This is well-defined since, for every $a\in |\cM_1|\cap|\cM_2|=|\cM_0|$, we have that $f^{\cM}(a):=f^{\cM_1}(a)=f^{\cM_0}(a)=f^{\cM_2}(a)$.  For every $n$-ry relation symbol $R$, we let $R^{\cM}$ be the union of $R^{\cM_1}\cup R^{\cM_2}$; notice that if the tuple $\ua$ belongs to $ R^{\cM}$, then we must have that  $\ua\in |\cM_i|^n$ and that $\ua\in R^{\cM_i}$ for either $i=1$ or $i=2$ (or for both, but this happens just in case $\ua\in |\cM_0|^n=|\cM_1|^n\cap |\cM_2|^n$). %because $\cM_0$ is a substructure of $\cM_1$ and $\cM_2$).
%
It is clear that $\cM_1$ and $\cM_2$ are substructures of $\cM$, and their inclusions agree on $\cM_0$.

We show that the $\Sigma$-structure $\cM$, as defined above, is a model of $T$. By hypothesis, $T$ is axiomatized by universal one-variable formulae: so, we can consider $T$ as a theory formed by axioms $\phi$ which are universal closures of clauses with just one variable, i.e. $\phi:=\forall x (A_1(x)\wedge...\wedge A_n(x)\rightarrow B_1(x)\vee...\vee B_m(x))$, where $A_j$ and $B_k$ ($j=1,...,n$ and $k=1,...,m$) are atoms.
%
We show that $\cM$ satisfies all such formulae $\phi$. In order to do that, suppose that, for every $a\in |\cM|$, $\cM\models A_j(a)$ for all $j=1,...,n$. If $a\in |\cM_i|$, then $\cM\models A_j(a)$ implies $\cM_i\models A_j(a)$, since $A_j(a)$ is a ground formula. Since $\cM_i$ is model of $T$ and so $\cM_i\models \phi$, we get that $\cM_i\models B_k(a)$ for some $k=1,...,m$, which means that $\cM\models B_k(a)$, since $B_k(a)$ is a ground formula. Thus, $\cM\models\phi$ for every axiom $\phi$ of $T$, i.e. $\cM\models T$ and, hence, $\cM$ is a $T$-amalgam of $\cM_1, \cM_2$ over $ \cM_0$, as wanted.
	
Now, given a primitive formula $\exists \ue \,\phi(\ue,\uy)$, we find a suitable $\psi(\uy)$ such that conditions {\rm (i)} and {\rm (ii)} of Lemma~\ref{lem:cover} hold. We define $\psi(\uy)$ as the conjunction of the set of all quantifier-free $\chi(\uy)$-formulae such that $\phi(\ue,\uy)\rightarrow \chi(\uy)$ is a logical consequences of $T$ (they are finitely many - up to $T$-equivalence - because $\Sigma$ is acyclic). By definition, clearly we have that {\rm (i)} of Lemma~\ref{lem:cover} holds.

By using amalgamation and the Robinson  Diagram Lemma, we show that also condition {\rm (ii)} of Lemma~\ref{lem:cover} is satisfied, as required.
 Let $\cM$ be a model of $T$ such that $\cM\models \psi(\ua)$ for some tuple of elements $\ua$ from the support of $\cM$. Then, consider the $\Sigma$-substructure $\cM[\ua]$ of $\cM$ generated by the elements $\ua$: this substructure is finite (since $\Sigma$ is acyclic), it is a model of $T$ and we trivially have that $\cM[\ua]\models \psi(\ua)$, since $\psi(\ua)$ is a ground formula. In order to prove that there exists an extension $\cN^{\prime}$ of $\cM[\ua]$ such that $\cN\models \exists \ue\,\phi(\ue,\ua)$, it is sufficient to prove (by the Robinson Diagram Lemma) that the $\Sigma^{|\cM[\ua]|\cup\{\ue\}}$-theory $\Delta(\cM[\ua])\cup\{\phi(\ue,\ua)\}$ is $T$-consistent. For reduction to absurdity, suppose that the last theory is $T$-inconsistent. Then, there are finitely many literals $l_1(\ua),..., l_m(\ua)$ from $\Delta(\cM[\ua])$  such that $\phi(e,\ua)\models_T \neg(l_1(\ua)\wedge...\wedge l_m(\ua))$. Therefore, defining $A(\ua):=l_1(\ua)\wedge...\wedge l_m(\ua)$, we get that $\phi(e,\ua)\models_T \neg A(\ua)$, which implies that $\neg A(\ua)$ is one of the $\chi(\uy)$-formulae appearing in $\psi(\ua)$. Since $\cM[\ua]\models \psi(\ua)$, we also have that $\cM[\ua]\models \neg A(\ua)$, which is a contradiction: in fact, by definition of diagram, $\cM[\ua]\models A(\ua)$ must hold. Hence, there exists an extension $\cN^{\prime}$ of $\cM[\ua]$ such that $\cN^{\prime}\models\exists \,\ue\phi(\ue,\ua)$.
Now, by amalgamation property, there exists a $T$-amalgam $\cN$ of $\cM$ and $\cN^{\prime}$ over $\cM[\ua]$: clearly, $\cN$ is an extension of $\cM$ and, since $\cN^{\prime}\hookrightarrow \cN$ and $\cN^{\prime}\models\exists \ue\,\phi(\ue,\ua)$, also $\cN\models\exists \ue\,\phi(\ue,\ua)$ holds, as required.
 \end{proof}
 
 

%\input{app1}

Since acyclicity of $\Sigma$ yields local finiteness, we immediately get as a Corollary the decidability of safety problems for transitions systems based on DB schema satisfying the hypotheses of the above theorem.  
	
 

